Les Houches 2013: Physics at TeV Colliders: Standard Model Working Group Report

This Report summarizes the proceedings of the 2013 Les Houches workshop on Physics at TeV Colliders. Session 1 dealt primarily with (1) the techniques for calculating standard model multi-leg NLO and NNLO QCD and NLO EW cross sections and (2) the comparison of those cross sections with LHC data from Run 1, and projections for future measurements in Run 2.

==> isolation/isolation-jpeg.tex <==


\section{Photon isolation studies \footnote{L.~Cieri and D.~de~Florian}}
%\section{Photon isolation studies \footnote{Leandro Cieri and Daniel de Florian}}



\subsection{INTRODUCTION}

Many interesting physics signatures at the LHC involve the presence of single or multiple photons in the final state. These photons may either be produced directly, through the fragmentation of a quark or gluon, or else through the decay of a resonance -- such as e.g. the Higgs boson.

The production of prompt photons is the subject of this analysis. The expression `prompt photons' refers to photons produced at large transverse momenta which do not arise from the decay of hadrons, such as $\pi^{0}$, $\eta$, etc. Prompt photons can be produced according to two possible mechanisms, one of them being fragmentation.

To be precise, the collider experiments at the Tevatron and the LHC do not perform {\it inclusive} photon measurements. The background of secondary photons coming from the decays of $\pi^{0}$, $\eta$, etc., overwhelms the signal by several orders of magnitude. To reject this background, the experimental selection of prompt diphotons requires {\em isolation} cuts. In addition to the rejection of the background of secondary  photons, the isolation cuts (or criteria) also affect the prompt-diphoton cross section itself, in particular by reducing the effect of fragmentation.

The standard cone isolation and the ``smooth'' cone isolation proposed by Frixione \cite{Frixione:1998jh} are two of these criteria. The standard cone isolation is easily implemented in experiments, but it only suppresses a fraction of the fragmentation contribution. The smooth cone isolation (formally) eliminates the entire fragmentation contribution, but its experimental implementation (at least in its original form) is complicated\footnote{There is activity in the experimental implementation~\cite{Binoth:2010ra,Blair:1379880,Wielers:2001suas} of the discretized version of the smooth isolation criterion. An experimental implementation of the smooth isolation criterion was done by the OPAL collaboration~\cite{Abbiendi:2003kf}.} by the finite granularity of the LHC and Tevatron detectors.

On the theoretical side, including fragmentation contributions to photon production can greatly increase the complexity of the calculations, while the application of appropriate isolation cuts can effectively remove those fragmentation contributions. How to apply these isolation criteria to the theoretical tools and how to deal with the fragmentation contributions consistently by the theory side is one of the subjects of this note.

Besides the differences between these two isolation criteria, it is possible (\textit{i.e.} it has physical meaning) to compare theoretical descriptions obtained using the smooth cone isolation criterion and data taken with the standard criterion, because a cross section obtained using the smooth cone isolation criterion provides always a lower bound for a cross section in which the standard criterion was implemented, if one uses the same isolation parameters for both criteria. Furthermore, as we show in this note, this bound turns out to be an excellent approximation to the standard criterion result with an accuracy of the order of the $1 \%$ if tight cuts are imposed.

Given these results, and the fact that in general it is not possible to exactly match the experimental isolation conditions to the theoretical implementation and viceversa,  we propose a pragmatic accord to perform a more precise comparison between the data and the fixed order calculations, that allows to extend the TH computation up to NNLO in some cases.
 That is the major motivation for this note.


The following studies concern Monte Carlo integrators (as {\small \texttt{DIPHOX}}~\cite{hep-ph:9911340}, {\small \texttt{JetFOX}}~\cite{hep-ph:0204023} or {\small \texttt{2$\gamma$NNLO}~\cite{Catani:2011dp}}, etc) for which the fragmentation component is a purely collinear phenomenon. For Monte Carlo generators (parton--shower Monte Carlo), in which the fragmentation photons are emited off quarks at non--zero angle during the showering process, we recomend reference~\cite{AlcarazMaestre:2012vp}.

 
\subsection{ISOLATION CRITERIA}
In this section we sumarize the standard and ``smooth'' isolation criteria, including their advantages and problems concerning the theoretical and experimental implementations.

\subsubsection{The standard cone isolation criterion}
The isolation criterion used by collider experiments is schematically as follows. A photon is said to be isolated if, in a cone of radius $R$ in rapidity and azimuthal angle around the photon direction, the amount of deposited hadronic transverse energy $\sum E_{T}^{had}$ is smaller than some value $E_{T \, max}$ chosen by the experiment:  
\begin{equation}\label{standardcriterion}     
\sum E_{T}^{had} \leq E_{T \, max} \;\;\;\; \mbox{inside} \;\;\;\;      
\left( y - y_{\gamma} \right)^{2} +    
\left(  \phi - \phi_{\gamma} \right)^{2}  \leq R^{2}  \;,    
\end{equation} 
where $E_{T \, max}$ can be either, a fixed value\footnote{This requirement was typically used at the Tevatron and was motivated by the fact that most of the energy in the isolation cone results from the underlying event (and pile-up), and so is independent of the photon energy~\cite{Binoth:2010ra}.} or a fraction of the transverse momentum of the photon ($p_T^{\gamma}\epsilon$, where typically $0 < \epsilon \leq 1$). This is the so-called standard cone isolation criterion. In addition to the rejection of the background of secondary  photons, these isolation cuts also affect the prompt-diphoton cross section itself, in particular by reducing the effect of fragmentation, but should be structured so as to have a high efficiency for the retention of real, isolated photons. 

A theoretical description of isolated photons is complicated because of the occurence of collinear singularities between photons and final-state quarks. A finite cross section is only obtained when these singularities are absorbed into the fragmentation functions. As a result the only theoretically well-defined quantity (if we don't use the smooth cone criterion) is the sum of the direct and fragmentation contributions. Once these two contributions are included one can isolate the photon using the cuts of Eq. (\ref{standardcriterion}) in an infrared safe way \cite{Catani:2002ny}.

In addition, a tight isolation cut also has the undesirable effect of making the theoretical prediction unstable~\cite{Catani:2002ny}, due to the restriction of the available phase-space for parton emission.  When the size of the cone used is in the limit of the narrow cone ($R\ll 1$, $R\sim 0.1$) earlier studies reveal potential problems. This leads to a collinear sensitivity in the form of a fairly large dependence on $\ln(1/R)$, which could make the prediction unreliable\footnote{This could even lead to an unphysical result such as an isolated cross section larger than the inclusive one, thereby violating
unitarity.}. In a recent calculation \cite{Catani:2013oma} these large logarithmic terms were ressumed restoring the reliability of the calculation.


\subsubsection{The ``smooth'' isolation criterion}
\label{Sec:Isol_Frix}
There exist an alternative to the standard criterion: the criterion proposed by Frixione in Ref.~\cite{Frixione:1998jh}
(see also Ref.~\cite{Frixione:1999gr,Catani:2000jh}). This criterion modifies Eq.~(\ref{standardcriterion}) in the following way
\begin{equation}\label{Eq:Isol_frixcriterion}     
\sum E_{T}^{had} \leq E_{T \, max}~\chi(r)\;, \;\;\;\; \mbox{inside any} \;\;\;\;      
r^{2}=\left( y - y_{\gamma} \right)^{2} +    
\left(  \phi - \phi_{\gamma} \right)^{2}  \leq R^{2}  \;.    
\end{equation}  
with a suitable choice for the function $\chi(r)$. This function has to vanish smoothly when its argument goes to zero ($\chi(r) \rightarrow 0 \;,\; \mbox{if} \;\; r \rightarrow 0\,$), and  has to verify \mbox{$\; 0<\chi(r)< 1$}, if \mbox{$0<r<R\,\,.$} One possible election is,
\begin{equation}
\label{Eq:Isol_chinormal}
\chi(r) = \left( \frac{1-\cos (r)}{1-\cos R} \right)^{n}\;,
\end{equation}
where $n$ is typically chosen as $n=1$ (unless otherwise stated we rely on this value for the phenomenlogical results presented in this note). This means that, closer to the photon, less hadronic activity is permitted inside the cone. At $r=0$, when the parton and the photon are exactly collinear, the energy deposited inside the cone is required to be exactly equal to zero, and the fragmentation component (which is a purely collinear phenomenon in perturbative QCD) vanishes completely. Since no region of the phase space is forbidden, the cancellation of soft gluon effects takes place as in ordinary infrared-safe cross sections. This is the advantage of this criterion: it eliminates all the fragmentation component in an infrared-safe way.

We can also notice, comparing Eqs.~(\ref{standardcriterion}) and (\ref{Eq:Isol_frixcriterion}), that both criteria coincide at the outer cone ($r=R$, $\chi(R)=1$), and due to the presence of the $\chi(r)$ function which verifies $0\leq\chi(r)\leq 1$, the smooth cone isolation criterion is more restrictive than the standard one. For this reason, we expect smaller cross sections when one uses the smooth cone criterion compared to the case when one implements the standard one if the same parameters are imposed,
\begin{equation}
\sigma_{smooth}\{R,E_{T~max}\}\leq \sigma_{Stand}\{R,E_{T~max}\}\,\,.
\end{equation}
The smooth behaviour of the $\chi(r)$ function is the main obstacle to implement the new isolation criterion into the experimental situation. First, because of the finite size of the calorimeter cells used to measure the electromagnetic shower, the smooth cone criterion must be applied only beyond a minimum distance of approximately $0.1$ (in $\{ \Delta \eta, \Delta \phi \}$ plane). This allows a contribution from fragmentation in the innermost cone and one has to check to which extent the fragmentation component is still suppressed. In addition, the transverse energy in the experimental isolation cone is deposited in discrete cells of finite size. Thus concerning its experimental implementation, the continuity criterion, initially proposed by Frixione has to be replaced by a discretized version consisting of a finite number of nested cones, together with the collection of corresponding maximal values for the transverse energy allowed inside each of these cones.

As was previously noted, another interesting (theoretical) feature of the smooth cone isolation criterion is that it is free of the large logarithmic contributions of the type of $\ln(1/R)$ associated with the narrow cone. 

%In particular a diphoton NLO cross section obtained with the Frixione isolation criterion in this narrow cone limit ($R\ll 1$, $R\sim 0.1$) remains smaller than the inclusive cross section.


\subsubsection{Theoretical issues}
%It is known at the theoretical level, there are specials cases in which the standard cone isolation criterion introduce instabilities and inconsistencies in the calculation.
%Here we will show that this criterion could introduce other undeaseable effects in the calculation if we don't include the fragmentation contribution in a consistent way.
As it was previously stated, the inclusion of the fragmentation contributions complicates the calculation. And in some cases, such as when one wants to reach NNLO accuracy in pQCD (like in diphoton production) it would make the calculation very unlikely for at least quite a few years since the machinary for such a computation is not available yet.


For those cases, one can find in the literature theoretical calculations in which the fragmentation component is considered at one pertubative level less than the direct component (\textit{e.g.} the $\gamma \gamma$ and $W/Z \gamma$ production at NLO in pQCD in {\small \texttt{MCFM}} \cite{Campbell:2011bn} or $\gamma \gamma +$ Jet at NLO in pQCD~\cite{Gehrmann:2013aga}, etc.). This procedure, which is a way to approximate the full calculation where the fragmentation component is included at the same perturbative level that the direct component, could introduce unexpected (inconsistent) results in the presence of the standard cone isolation criterion. The following  exercise shows how these problems can easely appear.

Let's consider diphoton production at the LHC ($\sqrt{s}=8$~TeV) computed at NLO, the highest perturbative order at which both direct and fragmentation calculations are available. The acceptance criteria in this case requires: $p_T^{\rm harder}\geq
40$~GeV and $p_T^{\rm softer}\geq 30$~GeV. The rapidity of both photons is restricted to \mbox{$|y_\gamma| \leq 2.5$} and $100$~GeV$<M_{\gamma \gamma}<160$~GeV. The isolation parameters are set to the values $n=1$ (in the case of the smooth cone) and $R=0.4$, and the minimum angular separation between the two photons is $R_{\gamma\gamma}=0.5$. The remain isolation parameter $E_{T~max}$ (or $\epsilon$) is varied in order to understand the cross section dependence on it. All the cross sections are obtained using the {\small \textsf{CTEQ6M}} set of parton distributions functions.
% , except for a few cases in which the different sets used are specified in detail. 
We used for this analysis the {\small \texttt{DIPHOX}} code that includes the full NLO pQCD description. 

First,  we compare the calculation using the fragmentation at NLO with the case in which the fragmentation is considered only at LO (one pertubative order less than the direct NLO component). The results in Fig. \ref{Fig:Isol_1} (right) show that for the LO fragmentation one can obtain 
larger cross sections for more severe isolation cuts (smaller $\epsilon$), which is clearly inconsistent. 
The same behaviour was reported in Ref.~\cite{Gehrmann:2013aga} for $\gamma \gamma +$ Jet at NLO, and we obtained similar features for $\gamma \gamma$, $W/Z \gamma$ production at NLO in pQCD with {\small \texttt{MCFM}}. 
On the other hand, the left panel in Fig. \ref{Fig:Isol_1} shows that the  correct behaviour is found when one considers the full result in which the fragmentation contribution is computed at same perturbative level than the direct component (i.e., NLO in this case).

The precedent comparison suggests that one has to be aware that approximating the fragmentation component at one order lower than the direct one can result in unphysical results. The situation can be even more serious when one looks at some extreme kinematical region where the cross section is dominated by higher order contributions. 
% This kind of unphysical behaviour is never found when the smooth cone isolation is imposed. 



\begin{figure}
\begin{center}
\includegraphics[width=0.48\textwidth,height=6.8cm]{NLONLO_LH_SinFrix_new}
\includegraphics[width=0.48\textwidth,height=6.8cm]{NLOnlo_LH_sinFrix}
 \caption{Diphoton cross section as a function of the invariant mass $M_{\gamma\gamma}$. (Left) With NLO fragmentation component. (Right) With LO fragmentation component.}
\label{Fig:Isol_1}
\end{center}
\end{figure}


In Table \ref{Tab:Isol_CMSNLO} we present the results for the corresponding cross section with different isolation prescriptions and parameters. The values presented there  help to understand the unexpected behaviour in Fig. \ref{Fig:Isol_1} (right). In this case, the results are obtained imposing the cuts used by CMS in a recent measurement of the production cross section for pairs of isolated photons in pp collisions at $\sqrt{s}=7$ TeV~\cite{Chatrchyan:2011qt}. Therefore, we require the harder photon to have a transverse momentum $p_T^{hard}\geq 40$ GeV while for the softer we choose $p_T^{soft}\geq 30$ GeV.
The rapidity of both photons is restricted to $|y_\gamma| \leq 2.5$. Finally, we constrain the invariant mass of the diphotons to lie in the range $100 \,{\rm GeV}\leq M_{\gamma\gamma} \leq 160\,{\rm GeV}$. And to simulate the CMS crack, we reject photons with  $1.442 \leq y_\gamma \leq 1.556$. In the cases in which the standard criterion was applied ($a-f$ in Table \ref{Tab:Isol_CMSNLO}) we observe that as the isolation criterion turns out to be ``loose'' the NLO direct component becomes smaller and the NLO fragmentation (single and double) component larger. The sum of them behaves as expected with respect to the isolation parameters, since the increase in the fragmentation component overcompensates the decrease of the direct  one. We remind the reader that in the standard isolation the theoretical separation between direct and fragmentation components is not physical and the results presented in this note correspond to the conventional $\overline{MS}$ subtraction.
On the other hand, if only the LO calculation is used for the fragmentation contributions, for which the QCD corrections are quite large (with $K-$factors exceding 2), the mismatch in the perturbative order spoils the compensation between the behaviour of the NLO direct and the LO fragmentation terms resulting in the unphysical behaviour observed in Fig. \ref{Fig:Isol_1} (right) as one considers less restringent isolation parameters.

Furthermore, from the cases in which the smooth cone criterion was applied ($h-m$ in Table \ref{Tab:Isol_CMSNLO}) we observed that, as expected, the result in the smooth cone case always provides a lower bound for the one obtained with the standard criterion when the same isolation parameters (energy in this case) are used. In the case of smooth cone isolation the (single and double) fragmentation components are identically null.
Even more interestingly, and with one single exception, the results for the NLO cross sections computed using different isolation precriptions differ by less than $1\%$. This result indicates that using the smooth cone prescription for a theoretical calculation (even when the data is analyzed using the standard one) provides an approximation that it is is far much better than the one consisting in the standard prescription with a lowest order calculation for the fragmentation component. 
The only case where one can observe larger differences (of the order of $10\%$) corresponds to the use a very loose isolation, as  for $\sum E_{T}^{had} \leq 0.5~p_{T}^{\gamma}$, where the fragmentation component in the standard case amounts more than half of the total cross section. 

\begin{table}[ht]
\begin{center}
\resizebox{14cm}{!} {
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
&Code & $\sum E_{T}^{had} \leq $& $\sigma_{total}^{NLO}$(fb)& $\sigma_{dir}^{NLO}$(fb) & $\sigma_{onef}^{NLO}$(fb)& $\sigma_{twof}^{NLO}$(fb)&Isolation\\%&Notes\\
\hline
\hline
a&\texttt{DIPHOX}& $2$ GeV & $3756$ & $3514$& $239$& $2.6$&Standard\\%&~\\
\hline
b&\texttt{DIPHOX}& $3$ GeV & $3776$ & $3396$& $374$& $6$&Standard\\%&~\\
\hline
c&\texttt{DIPHOX}& $4$ GeV & $3796$ & $3296$& $488$& $12$&Standard\\%&~\\
\hline
d&\texttt{DIPHOX}& $5$ GeV & $3825$ & $3201$& $607$& $17$&Standard\\%&~\\
\hline
e&\texttt{DIPHOX}& $0.05~p_{T}^{\gamma}$ & $3770$ & $3446$& $320$& $4$&Standard\\%&~\\
\hline
f&\texttt{DIPHOX}& $0.5~p_{T}^{\gamma}$ & $4474$ & $2144$& $2104$& $226$&Standard\\%&~\\
\hline
g&\texttt{DIPHOX}& \textit{ incl} & $6584$ & $1186$& $3930$& $1468$&none\\%&~\\
\hline
h&\texttt{2$\gamma$NNLO}& $0.05~p_{T}^{\gamma}~\chi(r)$ & $3768$ & $3768$& $0$& $0$&Smooth\\%&~\\
\hline
i&\texttt{2$\gamma$NNLO}& $0.5~p_{T}^{\gamma}~\chi(r)$ & $4074$ & $4074$& $0$& $0$&Smooth\\%&~\\
\hline
j&\texttt{2$\gamma$NNLO}& $2$ GeV~$\chi(r)$ & $3754$ & $3754$& $0$& $0$&Smooth\\%&~\\
\hline
k&\texttt{2$\gamma$NNLO}& $3$ GeV~$\chi(r)$ & $3776$ & $3776$& $0$& $0$&Smooth\\%&~\\
\hline
l&\texttt{2$\gamma$NNLO}& $4$ GeV~$\chi(r)$ & $3795$ & $3795$& $0$& $0$&Smooth\\%&~\\
\hline
m&\texttt{2$\gamma$NNLO}& $5$ GeV~$\chi(r)$ & $3814$ & $3814$& $0$& $0$&Smooth\\%&~\\
\hline
\hline

\end{tabular}

}
\end{center}
\caption{{\em Cross sections for the $pp\to \gamma\gamma+X$ process at the LHC at NLO.  All these values are at $1\%$ of statistical accuracy level.}}
\label{Tab:Isol_CMSNLO}
\end{table}








In all cases we have studied, the smooth cone provides an excellent approximation to the standard result as long as the isolation parameters are tight enough, i.e.  $\sum E_{T}^{had} \leq 0.1~p_{T}^{\gamma}$ or $\sum E_{T}^{had} \leq 5$ GeV for the LHC at 7 TeV. Equivalently, one could define the isolation to be tight enough when the contribution from the fragmentation component does not exceeds $\sim 15-20 \%$ of the total cross section.






\begin{figure}
\begin{center}
\includegraphics[width=0.48\textwidth,height=6.8cm]{CosTheta_Star_FRIX_FRAG_NLO_LO}
\includegraphics[width=0.51\textwidth,height=7.0cm]{D_Phi_FRIX_FRAG_NLO_LO}
 \caption{Diphoton cross section as a function of the $\cos \theta^{*}$ (Left), and  the angular separation between the photons $\Delta \phi_{\gamma \gamma}$ (Right). A comparison between the different isolation criteria is showed. The applied cuts are the same as in Fig. \ref{Fig:Isol_1}, and are described in the text.}
\label{Fig:Isol_2}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.48\textwidth,height=6.8cm]{Fig_3_Izq}
\includegraphics[width=0.48\textwidth,height=7.0cm]{Fig_3_Der}
 \caption{Diphoton cross section as a function of the invariant mass $M_{\gamma\gamma}$.  Cross sections obtained with the standard cone isolation criterion (with LO and NLO fragmentation contributions) are compared with the cross section obtained with the smooth cone criterion using the same isolation parameters.
}
\label{Fig:Isol_compToT}
\end{center}
\end{figure}
 

While the previous analysis refers only to the fiducial crosss section, it is known that the fragmentation contributions could be larger in kinematical regions far away from the back-to-back configuration\footnote{The low mass region in the invariant mass distribution, the low $\Delta \phi_{\gamma\gamma}$ distribution and the kinematical regions near to $\cos \theta^{*}=\pm 1$ belong to this case.}, and the approximation could in principle become less accurate for those distributions. In order to check that feature, in Fig. \ref{Fig:Isol_compToT} we compare the distributions for the full NLO calculation with the standard prescription, the one obtained using only the LO fragmentation component and the result for the smooth cone with $\sum E_{T}^{had} \leq 0.05~p_{T}^{\gamma}$  for $\cos \theta^{*}$ (left) and $\Delta \phi_{\gamma\gamma}$ (right). In both cases we observe that for all the bins the smooth cone provides the best approximation to the full result, always within a $2.5 \%$ accuracy. A more detailed analysis in presented in Fig. \ref{Fig:Isol_compToT} for the diphoton invariant mass distributions with two different isolation parameters, $\sum E_{T}^{had} \leq 0.05~p_{T}^{\gamma}$ (left) and $\sum E_{T}^{had} \leq 4$ GeV (right). Again, while using the LO fragmentation component fails to reproduce the full NLO result by up to $6\%$, the smooth cone approximation is always better than $1.5\%$ in the same kinematical region.



The discrepancies between the full result and the smooth approach with the LO fragmentation approximation that evidently manifest in the invariant mass distribution (see Fig. \ref{Fig:Isol_compToT}) or in kinematical regions far away from $\cos \theta^{*}=\pm 1$ (see Fig. \ref{Fig:Isol_2} (left)) are ``hidden'' in the $\Delta \phi_{\gamma\gamma}$ distribution, in the bin corresponding to $\Delta \phi_{\gamma\gamma}=\pi$ (the bin containing the back-to-back configurations). Moreover in the low $\Delta \phi_{\gamma\gamma}$ region   we are dealing with events far away from the back-to-back configuration, and the only configuration that survives at NLO (in these kinematical regions) is the real emission at LO which is for the three cases effectively the same contribution under these conditions. 



\begin{figure}
\begin{center}
\includegraphics[width=0.50\textwidth,height=6.8cm]{D_Phi_FRAG_NLO_LO_FRIX_eps_1}
\includegraphics[width=0.46\textwidth,height=6.8cm]{Mgg_FRIX_FRAG_NLO_LO_eps_1}
 \caption{Diphoton cross section as a function of the angular separation between the photons $\Delta \phi_{\gamma\gamma}$ (Left), and  the invariant mass of the diphoton system $M_{\gamma\gamma}$ (Right).}
\label{Fig:Isol_3}
\end{center}
\end{figure}


If one relaxes the isolation and considers $\epsilon =1$ (which is equivalent to $E_{T}^{max}>40$~GeV, allowing for a huge amount of fragmentation contribution), the effects of fragmentation now  strongly manifests at low $\Delta \phi_{\gamma\gamma}$ values, and the full result considerably differs from both the LO fragmentation approximation and the smooth cone criterion as we can observe in Fig. \ref{Fig:Isol_3} (azimuthal distribution in the upper plot and invariant mass in the lower one). Also we can see from Fig. \ref{Fig:Isol_3}, in the bin corresponding to $\Delta \phi_{\gamma\gamma}=\pi$ (the bin containing the back-to-back configurations) the cross section obtained with the smooth cone criterion provides a better approximation  than the LO fragmentation one. 





\subsection{Tight isolation accord}
Finally, considering the results presented in the preceeding sections we conclude this note by proposing a pragmatic accord in order to compare experimental data and theoretical calculations obtained at the highest possible perturbative order. Given the fact that matching experimental conditions to theoretical calculations always implies certain degree of approximation, we believe that considering the large QCD corrections to processes involving photons (with NNLO essential to understand diphoton data~\cite{Catani:2011dp}) and the agreement (tipically at the $\%$ level for the diphoton case studied here) between the standard and smooth cone TH calculations, the use of the later for TH purposes is well justified.

We call this approach "pragmatic", in the sense that we do not recommend the experiments to implement the smooth cone isolation, but to proceed to the analysis of the data with the usual standard isolation with cuts tight enough if the interesting observable needs to be an isolated cross section or distribution.
While the definition of "tight enough" might slightly depend on the particular observable (that can always be checked by a lowest order calculation), our analysis shows that at the LHC isolation parameters as $E_{T}^{max}\leq 5$~GeV (or $\epsilon<0.1$), $R\sim 0.4$ and $R_{\gamma\gamma}\sim 0.4$ are safe enough to proceeed.

This procedure would allow to extend available NLO calculations to one order higher (NNLO) for a number of observables, since the direct component is always much simpler to evaluate than the fragmentation part, which identically vanishes under the smooth cone isolation.

We also refer to this approach as pragmatic in a numerical sense: we are certain that the smooth cone isolation applied for the TH calculation is NOT the one used in the experimental data, but considering that NNLO corrections are of the order of $50\%$ for diphoton cross sections~\cite{Catani:2011dp} and a few $100\%$ for some distributions in extreme kinematical configurations, it is far better accepting a few $\%$ error arising from the isolation (less than the size of the expected NNNLO corrections and within any estimate of TH uncertainties!) than neglecting those huge QCD effects towards some "more pure implementation" of the isolation prescription.

We believe that a more detailed analysis of the profile function in the smooth cone isolation can be performed on a case by case basis in order to select, also in a pragmatic way, the most convenient for each observable, even though again, differences are expected to be very small as discussed before.




\subsection*{ACKNOWLEDGEMENTS}
This work was supported in part by UBACYT, CONICET, ANPCyT, INFN and the Research Executive Agency (REA) of the European Union under the Grant Agree- ment number PITN-GA-2010-264564 (LHCPhenoNet, Initial Training Network).


\bibliography{isolation}




